TITAN: Twin-Informed Topology Adaptation for LAWN-enabled D2C Communication

Low-Altitude Wireless Networks (LAWN) are transforming the low-altitude airspace into a mission-driven, dynamically reconfigurable 3D network fabric for safety-critical and public-safety operations. In parallel, Direct-to-Cell (D2C) satellite access can rapidly restore connectivity after disasters, yet dense urban blockages make the satellite-to-ground link unreliable for many users. To overcome this, we leverage the LAWN aerial layer and form an adaptive low-altitude relay topology where Unmanned Aerial Vehicles (UAVs) act as D2C-assisted aerial relays for obstructed ground users. We introduce TITAN, a twin-informed topology adaptation framework that builds a high-fidelity Digital Twin (DT) of the affected urban area and performs site-specific, ray-traced air-to-ground channel modeling via Sionna RT. This informs a Bayesian optimization process that adapts the aerial topology to maximize coverage and Quality of Service (QoS) for ground users by using UAVs as optimal D2C relays. Extensive system-level simulations with Sionna show that TITAN consistently outperforms the baselines and delivers +32.2% user coverage, +64.9% system sum-rate, and +49.3% fairness over the state-of-the-art (SOTA) that employ heuristic placement or statistical channel approximations. To support further research in resilient network design, we open-source the codebase of the TITAN framework.

==> figures/Sources/intro_figure.tex <==
https://drive.google.com/file/d/1-MeDl0Q08IdEtCKpB5LRywtDVHjBoxQG/view?usp=sharing

==> notes.tex <==
Benefits
Here are some primary benefits of federated machine learning:
FL enables devices like mobile phones to collaboratively learn a shared prediction model while keeping the training data on the device instead of requiring the data to be uploaded and stored on a central server.
Moves model training to the edge, namely devices such as smartphones, tablets, IoT, or even “organizations” like hospitals that are required to operate under strict privacy constraints. Having personal data remain local is a strong security benefit.
Makes real-time prediction possible, since prediction happens on the device itself. FL reduces the time lag that occurs due to transmitting raw data back to a central server and then shipping the results back to the device.
Since the models reside on the device, the prediction process works even when there is no internet connectivity.
FL reduces the amount of hardware infrastructure required. FL uses minimal hardware and what is available in mobile devices is more than enough to run the FL models.


Challenges
There are a number of core challenges associated with FL. First, communication is a critical bottleneck in FL networks where data generated on each device remain local. In order to train a model using data generated by the devices in the network, it is necessary to develop communication-efficient methods that reduce the total number of communication rounds, and also iteratively send small model updates as part of the training process, as opposed to sending the entire data set.
Additionally, FL methods must: anticipate low levels of device participation, i.e. only a small fraction of the devices being active at once; tolerate variability in hardware that affects storage, computational, and communication capabilities of each device in a federated network; and be able to handle dropped devices in the network.
Finally, FL helps to protect data generated on a device by sharing model updates such as gradient data instead of raw data. But communicating model updates throughout the training process can still reveal sensitive information, either to a third party, or to the central server.




assumption:
origin for coordinates = 42.338128661705255, -71.08705289706138
BS coordinates = 42.33783671678225, -71.08665391849328


BS coordinates at new axis = 
32.7687648776171 -32.43832477769123

#cat1
('outshape', (9739, 2), (9739, 360, 640, 3), (9739, 20, 20, 20), (9739, 64))




% througput_ratio 0.8655079514890919
% latest_model = keras.models.load_model('/home/batool/FL/federated/models_portion2/global_model_round_29.h5',custom_objects={'top_2_accuracy':top_2_accuracy,'top_5_accuracy':top_5_accuracy,'top_10_accuracy':top_10_accuracy,'top_25_accuracy':top_25_accuracy,'top_50_accuracy':top_50_accuracy},compile=False)



%Inference_time 1627569192.3812978-1627569190.356182 
%# of sample is 3287 
% Inferen per sample is 0.00061609848 ~ 0.6 ms


%sending 7 bits on the channel with rate: 0.004 micro sec ~ 4 ns



% maximum FL accuracy= 0.68177
% througput_ratio 89.32328497583865

% 0.98610467809 decrease in time overhead
%0.5275 new correct time


% ########
% print(max(acc_all))% 0.67295

% print(max(acc_p1))% 0.66109

% print(max(acc_p2))% 0.6693000000000001

% print(max(acc_pgg))% 0.66474

% print(max(acc_pgl))% 0.6817799999999999




==> sections/unused/experimental-analysis-DR.tex <==
\section{PERFORMANCE EVALUATION}
In this section, we present a comprehensive performance evaluation of the TITAN framework based on the methodology outlined in Section V. We conduct a series of targeted experiments designed to validate TITAN's core contributions, analyzing its performance against established baselines and testing its robustness under non-ideal conditions. All results are averaged over 20 independent simulations with random UT distributions to ensure statistical significance.

\subsection{Scenario 1: Baseline Performance in Full Infrastructure Collapse}
This initial experiment evaluates the fundamental effectiveness of TITAN by simulating a worst-case disaster scenario where all three terrestrial gNBs have failed. This allows us to directly measure the benefits of TITAN's high-fidelity modeling (C1) and its efficient topology optimization (C2) in enabling D2C communication from a clean slate. We compare TITAN against the three baseline methods: Traditional D2C, Random UAV Placement, and Bayesian Optimization using the stochastic 3GPP TR38.901 model.

The results for sum-rate and coverage ratio as a function of the number of deployed UAVs are presented in Fig. 5 and Fig. 6, respectively. The Traditional D2C baseline, which does not use UAVs, is shown as a dashed line for reference.

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/performance/sum_rate.pdf}
        \caption{Sum-rate comparison.}
        \label{fig:qos_sumrate}
    \end{subfigure}
    % \hspace{-15pt}
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/performance/coverage_ratio.pdf}
        \caption{Coverage ratio comparison.}
        \label{fig:qos_coverage}
    \end{subfigure} 
    \caption{Sum-rate performance comparison in a full infrastructure collapse scenario. TITAN's use of a high-fidelity DT for optimization enables it to find superior UAV placements that significantly outperform all baselines.}
    \label{fig:sum_rate_baseline}
\end{figure}

\begin{figure}[!t]
    \centering
    % In your final paper, replace this placeholder with your actual figure file
    \includegraphics[width=0.24\textwidth]{figures/results/performance/fairness_index.pdf}
    \caption{Coverage ratio comparison in a full infrastructure collapse scenario. TITAN consistently achieves the target coverage ratio of 80\% with the minimum number of UAVs, unlike the baselines which struggle to provide reliable service.}
    \label{fig:coverage_baseline}
\end{figure}

\textbf{Observation 1:} The TITAN framework dramatically outperforms all baseline methods. The Traditional D2C approach provides negligible coverage and throughput, confirming its non-viability in urban canyons. While adding UAVs helps, the Random Placement strategy is highly inefficient. The Bayesian (TR38.901) baseline, which uses an intelligent optimizer but an inaccurate channel model, performs better but is still significantly surpassed by TITAN. With three UAVs, TITAN achieves a [40\%] higher sum-rate and provides [25\%] more coverage than the next-best approach, validating the critical importance of DT-informed, site-specific optimization (C1, C2).

\subsection{Scenario 2: Dynamic Adaptation to Partial Failures}
This experiment is designed to validate TITAN's ability to reactively adapt its topology to a dynamic disaster environment (C3). The simulation begins with all three terrestrial gNBs active, providing baseline coverage. We then simulate cascading failures by disabling the gNBs one by one. After each failure, TITAN is triggered to re-optimize and deploy an aerial topology to restore service.

Fig. 7 illustrates the network's performance throughout this process. It shows the initial sum-rate with all gNBs active, the performance drop after each failure, and the subsequent recovery achieved by TITAN's adaptive UAV deployment.

\begin{figure}[!t]
    \centering
    % In your final paper, replace this placeholder with your actual figure file
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/fidelity/sum_rate.pdf}
        \caption{Sum-rate versus fidelity level.}
        \label{fig:sum_fidelity}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/fidelity/coverage_ratio.pdf}
        \caption{Coverage ratio versus fidelity level.}
        \label{fig:cov_fidelity}
    \end{subfigure}
    \caption{Network performance during a cascading gNB failure scenario. The bars show the drop in sum-rate as gNBs fail and the subsequent recovery after TITAN adaptively deploys its aerial topology to compensate for the loss.}
    \label{fig:partial_failure}
\end{figure}

\textbf{Observation 2:} TITAN demonstrates highly effective reactive adaptation. After the first gNB fails, TITAN's deployment of a single UAV restores over [90\%] of the original network sum-rate. As more gNBs fail, TITAN continues to compensate by deploying additional UAVs, successfully maintaining a high level of service continuity. This validates the framework's ability to dynamically adapt to evolving on-the-ground conditions (C3).

\subsection{Scenario 3: Robustness to Imperfect Digital Twin}
This final set of experiments evaluates TITAN's resilience to the inevitable imperfections of a real-world deployment, directly validating its robustness (C4).

\subsubsection{Impact of UT Location Error}
We simulate the effect of inaccurate GPS data by adding Gaussian noise to the UT locations used during the optimization phase. Fig. 8 and Fig. 9 show the degradation in coverage ratio and sum-rate, respectively, as the location error increases from 0m (perfect knowledge) to 10m.

\begin{figure}[!t]
    \centering
    % In your final paper, replace this placeholder with your actual figure file
    \includegraphics[width=0.9\columnwidth]{figure_placeholder.png} 
    \caption{Impact of UT location error on the final coverage ratio achieved by TITAN's optimized topology. Performance remains high even with significant location uncertainty.}
    \label{fig:coverage_error}
\end{figure}

\begin{figure}[!t]
    \centering
    % In your final paper, replace this placeholder with your actual figure file
    \includegraphics[width=0.9\columnwidth]{figure_placeholder.png} 
    \caption{Impact of UT location error on the final sum-rate achieved by TITAN's optimized topology. The degradation is marginal, highlighting the robustness of the solution.}
    \label{fig:sum_rate_error}
\end{figure}

\textbf{Observation 3:} TITAN's topology optimization is highly robust to UT location errors. Even with a 10-meter standard deviation in location uncertainty—a significant error margin—the final sum-rate and coverage ratio degrade by less than [8\%]. This resilience is because the optimized high-altitude UAV positions create broad coverage footprints that inherently tolerate minor inaccuracies in ground user locations, proving TITAN's suitability for practical deployment (C4).

\subsubsection{Impact of DT Fidelity}
We investigate the trade-off between model accuracy and computational cost by running TITAN's optimization using a "Low-Fidelity" DT (e.g., maximum of 2 ray bounces) and comparing its final performance against an optimization run with a "High-Fidelity" DT (8 ray bounces). Both resulting topologies are evaluated in the high-fidelity environment.

\textbf{Observation 4:} Optimizing with a lower-fidelity DT provides a significant reduction in computational time per optimization iteration (over [4x] faster) while still achieving over [90\%] of the sum-rate performance of a full-fidelity optimization. This demonstrates that TITAN can be configured to provide a strong, near-optimal solution even under tight computational constraints, further underscoring its practical robustness (C4).

==> sections/unused/introduction-DR.tex <==
\section{Introduction DR}
{\color{teal}
\noindent{\bf The Criticality of Post-Disaster Communication.}
In the immediate aftermath of natural or man-made disasters, the single most critical asset for an effective response is a functioning communication network. The ability to dispatch first responders, issue public safety alerts, assess damage, and connect separated families is entirely dependent on the flow of information \cite{ali2021review}. However, the very infrastructure we rely on is often the first casualty. Disasters can cause widespread power outages, sever fiber optic backhaul lines, and physically destroy cellular base stations. This collapse of terrestrial networks creates a perilous information vacuum, severely hampering situational awareness and complicating rescue efforts at a time when coordination is paramount \cite{anjum2023space}. The urgent need for rapidly deployable, resilient, and high-performance communication solutions to operate in these contested environments has never been greater.

\noindent{\bf The Promise and Peril of Direct-to-Cell (D2C) Connectivity.}
A transformative technology poised to address this challenge is Direct-to-Cell (D2C) communication, which connects standard user devices directly to Low Earth Orbit (LEO) satellite constellations. This paradigm offers the revolutionary potential for near-instantaneous service restoration over vast areas without any reliance on local ground infrastructure. However, while D2C is effective in open rural areas, its viability in dense urban environments, where a significant portion of the population resides, is severely compromised. The satellite-to-ground link requires a clear Line-of-Sight (LoS) or near-LoS path, \textit{but in urban canyons,} this path is almost always obstructed by buildings and other structures, as illustrated in Fig. \ref{fig:d2c}. The steep elevation angles required to connect with LEO satellites mean that signals must penetrate multiple walls or be perfectly reflected, leading to crippling attenuation, polarization mismatch, and multipath fading that render the D2C link unusable for most ground-level users \cite{chen2020vision}.

\noindent{\bf From Architectural Solution to an Adaptation Problem: The Role of SAGINs and Digital Twins.}
To bridge this critical gap, an architectural solution is needed: a Space-Air-Ground Integrated Network (SAGIN) \cite{liu2018space}. Within a SAGIN, the aerial layer, comprised of agile assets like Unmanned Aerial Vehicles (UAVs), can serve as an on-demand relay network. A UAV  can maintain a strong and stable LoS backhaul link to an overhead satellite and then relay that connection to users on the ground, effectively circumventing the urban blockages that plague D2C. This SAGIN-enabled D2C model fundamentally reframes the problem. The question is no longer about the static availability of a link but about the dynamic deployment of an adaptive network topology. The challenge becomes one of intelligence and optimization: How can we autonomously place the UAVs to form the most effective relay topology in a complex, unpredictable, and partially destroyed environment?

This intelligent placement is impossible without a deep, site-specific understanding of the radio propagation environment. Conventional network planning tools, which rely on overly-simplified stochastic channel models, are inadequate. They average out the very deterministic, location-specific blockages and reflections that define the urban channel, leading to grossly inaccurate performance predictions and a suboptimal, unreliable aerial topology. To solve this, we must transition from statistical guesswork to deterministic prediction. This necessitates a high-fidelity Digital Twin (DT), as it enables precise environmental modeling and accurate performance forecasting for any candidate network configuration.

% \begin{figure}[!t]
%     \centering
%     % It's recommended to have a high-quality PDF/EPS for your figures
%     \includegraphics[width=\columnwidth]{figure_placeholder.png} 
%     \caption{The TITAN framework. A Digital Twin of the disaster scenario is created using environmental mesh data and user terminal (UT) locations. This enables precise ray-traced channel modeling to find the optimal adaptive aerial topology via Bayesian optimization, maximizing coverage and QoS.}
%     \label{fig:concept}
% \end{figure}

\noindent{\bf Key Research Challenges.}
Implementing a DT-informed framework for adaptive topology control requires overcoming several significant research challenges:

\begin{itemize}
    \item \textbf{(Ch1) High-Fidelity and Efficient Channel Modeling:} How can we accurately model the site-specific wireless channels across a large urban area? The modeling approach must capture deterministic effects like reflection and diffraction yet remain computationally efficient enough to be used within a real-time optimization loop.
    \item \textbf{(Ch2) Complex and High-Dimensional Topology Optimization:} How do we efficiently find the optimal number and 3D coordinates for a fleet of UAVs? The search space for this problem is vast, continuous, and high-dimensional. Furthermore, the objective function—overall network performance—is a "black box" that can only be evaluated through computationally expensive ray-tracing simulations, rendering brute-force or exhaustive search methods infeasible.
    \item \textbf{(Ch3) Proactive Adaptation to Environmental Dynamics:} How can the aerial topology dynamically adapt to the fluid nature of a disaster scenario? A truly resilient network must not only react to current conditions but also proactively reconfigure its topology to support predictable changes, such as the synchronized movement of first responders or evacuees along known routes.
    \item \textbf{(Ch4) Ensuring Robustness to Real-World Imperfections:} How will the optimized topology perform given the inevitable uncertainties of a real-world deployment? A practical framework must demonstrate robustness against imperfections such as noisy or outdated GPS data for ground users and varying levels of fidelity in the Digital Twin itself.
\end{itemize}

\noindent{\bf Our Proposed Solution: The \name~Framework.}
To address these multifaceted challenges, this paper introduces \textbf{\name}, a Twin-Informed Topology Adaptation framework for SAGIN-enabled D2C communication. At its heart, \name~ leverages a high-fidelity Digital Twin constructed from 3D environmental data (e.g., city mesh models) and the last known locations of users. By creating this virtual replica, \name~ replaces inaccurate stochastic models with precise, deterministic ray-traced channel simulations powered by Sionna RT, directly addressing (Ch1). This accurate channel knowledge becomes the input to a powerful Bayesian optimization engine, which intelligently and efficiently explores the high-dimensional search space to find a near-optimal aerial topology without requiring an exhaustive search, thus solving (Ch2). The framework is designed to be dynamic, incorporating predictive models to proactively reconfigure the topology in response to user mobility (Ch3). Finally, we rigorously test the entire system under a variety of imperfect conditions to validate its real-world robustness (Ch4).

\noindent{\bf Summary of Contributions.}
The primary contributions of this work are as follows:

\begin{enumerate}
    \item \textbf{(C1) High-Fidelity SAGIN Modeling Framework:} We design and implement a novel Digital Twin framework that integrates a state-of-the-art ray-tracing engine (SionnaRT) with a full 5G NR-compliant system-level simulator. This provides an end-to-end tool for accurately modeling and evaluating the performance of adaptive SAGIN topologies in complex, realistic urban environments.
    \item \textbf{(C2) Efficient Bayesian-based Topology Optimization:} We formulate the aerial network design as a complex, black-box optimization problem. We then solve it efficiently using Bayesian optimization to jointly determine the optimal number and 3D locations of UAVs, maximizing a composite utility function of network coverage, total capacity, and user fairness.
    \item \textbf{(C3) Proactive Mobility-Aware Adaptation Strategy:} We introduce and evaluate a proactive adaptation strategy that goes beyond simple reactive placement. By using a linear predictor to anticipate the trajectories of moving user groups, \name~ can pre-position aerial relays to ensure seamless service continuity and maintain high QoS during movement.
    \item \textbf{(C4) Comprehensive Robustness Analysis:} We conduct an extensive evaluation of \name's performance under non-ideal, real-world conditions. We demonstrate the framework's resilience to significant uncertainties, including errors in user location data and the trade-offs between Digital Twin fidelity and computational cost.
    \item \textbf{(C5) Open-Source Framework for Community Research:} We are releasing our entire Sionna-based simulation framework as an open-source tool. This contribution enables reproducible research and provides the community with a powerful platform for developing and testing new algorithms for network adaptation, as well as for generating large-scale datasets (e.g., channel impulse response, IQ samples) to train future data-driven and ML-based solutions.
\end{enumerate}
}

% When natural or man-made disasters strike, the collapse of terrestrial communication infrastructure severely hampers rescue and relief efforts. The ability to coordinate first responders, locate survivors, and inform affected populations hinges on restoring connectivity swiftly and reliably \cite{ali2021review}. In these critical moments, traditional cellular networks often fail due to physical damage to towers, power outages, or backhaul disruption, creating an information vacuum that can exacerbate the crisis \cite{anjum2023space}. This foundational problem underscores the urgent need for resilient communication paradigms that can be rapidly deployed in the most challenging environments.

% A promising solution is the advent of Direct-to-Cell (D2C) services, which aim to connect standard user terminals directly to Low Earth Orbit (LEO) satellites. This approach bypasses the need for local terrestrial infrastructure, offering the potential for near-instantaneous, wide-area coverage. However, the promise of D2C faces a fundamental obstacle in the very environments where disasters often occur: dense urban areas. As illustrated in Fig. \ref{fig:intro}, the satellite-to-ground link is highly susceptible to blockage by buildings, foliage, and terrain. This "urban canyon" effect means that for a vast majority of ground-level users, a reliable Line-of-Sight (LoS) path to a satellite is non-existent, rendering D2C communication ineffective when it is needed most \cite{chen2020vision}.

% To overcome the limitations of D2C, we can leverage the inherent flexibility of a multi-layered architecture, forming a Space-Air-Ground Integrated Network (SAGIN) \cite{liu2018space}. In a SAGIN, the aerial layer—composed of assets like Unmanned Aerial Vehicles (UAVs)—can act as an agile, on-demand relay network. By establishing a robust LoS backhaul link to a LEO satellite, a UAV can then relay the signal to obstructed users on the ground, effectively bypassing the urban blockages. This SAGIN-enabled D2C model transforms the problem from one of static link availability to one of dynamic network deployment. The central question is no longer {\em if} a connection is possible, but rather {\em how} to intelligently deploy the aerial assets to create the most effective and resilient communication topology.

% This leads to the core motivation for our work: making SAGIN-enabled D2C a practical reality requires a framework for intelligent, environment-aware topology adaptation. Simply deploying UAVs is not enough; their performance is entirely contingent on their precise 3D placement relative to the users and the surrounding environment. Conventional network planning, which relies on simplified, stochastic channel models, is ill-suited for this task. Such models fail to capture the deterministic, site-specific blockages and reflections that define the urban propagation landscape, leading to inaccurate performance predictions and a suboptimal, unreliable aerial topology. To truly optimize the network, we need a mechanism that can ``see'' the environment in high fidelity and predict the performance of any given UAV placement with precision. This is the role of a Digital Twin (DT).

% However, designing and implementing a DT-informed framework for adaptive topology control presents several significant challenges:

% \begin{itemize}
%     \item \textbf{(C1) Channel Modeling in Complex Environments:} How can we accurately and efficiently model the wireless channels in a complex, non-uniform urban environment? The model must be precise enough to capture site-specific effects but computationally tractable enough to be used within an optimization loop.
%     \item \textbf{(C2) High-Dimensional Topology Optimization:} How do we find the optimal number and 3D locations of UAVs? The search space for this problem is vast and continuous, and the objective function (i.e., network performance) is a ``black box'' that can only be evaluated through computationally expensive simulations, making exhaustive search impossible.
%     \item \textbf{(C3) Proactive Adaptation to Dynamics:} How can the aerial topology adapt to the dynamic nature of a disaster scenario? The framework must not only react to current conditions but also proactively reconfigure itself in response to predictable changes, such as the collective movement of evacuees or first responders.
%     \item \textbf{(C4) Robustness to Real-World Imperfections:} How does the system perform with imperfect information? A practical framework must be robust to real-world uncertainties, such as errors in the known locations of ground users or limitations in the fidelity of the Digital Twin itself.
% \end{itemize}

% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=0.99\linewidth]{figures/intro_scheme.pdf}
% %     \caption{The \name framework. A Digital Twin of the disaster scenario is created using environmental mesh data and user terminal (UT) locations. This enables precise ray-traced channel modeling to find the optimal adaptive aerial topology via Bayesian optimization, maximizing coverage and QoS.}
% %     \label{fig:concept}
% % \end{figure}

% To address these challenges, we propose \textbf{\name}, a Twin-Informed Topology Adaptation framework for SAGIN-enabled D2C communication. \name's core is a high-fidelity Digital Twin of the disaster zone, constructed from 3D environmental data and the last known locations of users. By creating this virtual replica, \name~replaces inaccurate stochastic models with precise, deterministic ray-traced channel simulations powered by SionnaRT (addressing C1). This environment-aware channel knowledge is then fed into a Bayesian optimization engine, which efficiently finds a near-optimal aerial topology without requiring an exhaustive search (addressing C2). The framework is designed to be dynamic, allowing for proactive reconfiguration based on predicted user mobility (addressing C3), and its performance is rigorously evaluated under imperfect conditions to ensure real-world viability (addressing C4).

% The main contributions of this paper are as follows:
% \begin{enumerate}
%     \item We design a novel Digital Twin framework that integrates realistic 3D environmental data with system-level simulations to accurately model the performance of a SAGIN's adaptive aerial layer in complex urban environments.
%     \item We formulate the aerial topology adaptation as a joint UAV count and placement optimization problem, which we solve efficiently using Bayesian optimization to maximize a composite utility of coverage, capacity, and fairness.
%     \item We introduce a proactive adaptation strategy that anticipates user mobility, allowing the aerial topology to be reconfigured ahead of time to ensure service continuity.
%     \item We demonstrate the robustness of \name~by evaluating its performance across varying levels of DT fidelity and UT location uncertainty, proving its efficacy for real-world deployment.
%     \item We are releasing our Sionna-based simulation framework as open-source, providing a tool for reproducible research and data collection (CIR, IQ samples) to foster innovation in adaptive network design.
% \end{enumerate}

==> sections/unused/system_model.tex <==
\section{System Architecture}
\label{system_model}
{\color{gray}}
\subsection{Digital Twin Channel Modeling}

In this work, wireless channels between UAV-mounted gNodeBs and user terminals (UTs) are modeled using deterministic ray tracing within the Digital Twin (DT) framework. Ray tracing enables precise characterization of multipath propagation by explicitly computing all significant signal trajectories (direct, reflected, diffracted, and scattered) between each transmitter-receiver pair, based on the geometric and electromagnetic properties of the environment. Given a 3D urban scene model, the Sionna engine systematically traces rays from each UAV antenna element to each UT, calculating the contribution of each path to the total received signal as a discrete tap with a specific delay and complex amplitude. This method yields a frequency-selective, time-dispersive channel model whose taps directly correspond to physical propagation mechanisms in the modeled environment. The resulting channel impulse responses (CIRs) serve as the foundation for all subsequent link-level and system-level simulations. The mathematical formulation of the modeled channel is provided below.

Each UT–gNodeB link is represented by a frequency-selective multipath propagation channel. The coherent CIR for UT $u$ from UAV gNodeB $b$ is expressed as a sum of discrete multipath taps:
\begin{equation}
    h_{u,b}(t) = \sum_{\ell=1}^{L_{u,b}} \alpha_{\ell,u,b}\,\delta(t - \tau_{\ell,u,b}),
\end{equation}
where $L_{u,b}$ denotes the number of taps between UT $u$ and UAV $b$, $\alpha_{\ell,u,b}$ represents the coherent complex amplitude, and $\tau_{\ell,u,b}$ is the delay of the $\ell$-th tap.

The path solver computes all channel taps simultaneously for each TX-RX antenna pair, forming a tensor representation. Considering $K$ transmitters, $M$ receivers, $Q$ antennas per transmitter, and $T$ antennas per receiver, the CIR is stored in a flexible tensor form accommodating variable-length taps:
\begin{align}
    \mathbf{H} = \Big\{\, 
    &\big\{\big(\alpha_{\ell,k,m,q,t},\;\tau_{\ell,k,m,q,t}\big)\big\}_{\ell=1}^{L_{k,m,q,t}} 
    \;:\nonumber\\
    &k\in[1,K],\; m\in[1,M],\; q\in[1,Q],\; t\in[1,T]
    \Big\}
\end{align}
where each entry contains a variable-length set of taps.

From the coherent CIR, the received signal power at UT $u$ from UAV $b$ is computed as the coherent sum across taps:
\begin{equation}
    P_{u,b} = \left|\sum_{\ell=1}^{L_{u,b}}\alpha_{\ell,u,b}\right|^2.
\end{equation}

The coherent SINR for UT $u$ associated with UAV $b$, given UAV placement configuration $\mathbf{X}$, is:
\begin{equation}
    \gamma_{u,b}(\mathbf{X}) = \frac{P_{u,b}}{\sum_{b'\neq b}P_{u,b'} + N_0},
\end{equation}
where $N_0$ is the noise power.

UT $u$ is declared \textit{covered} if its SINR surpasses a threshold $\gamma_{\text{th}}$:
\begin{equation}
    u \in \mathcal{U}_{\text{cov}}(\mathbf{X}) \iff \gamma_{u,b}(\mathbf{X}) \geq \gamma_{\text{th}}.
\end{equation}

\subsection{UAV Placement Optimization via Bayesian Techniques}
Due to computational complexity constraints associated with detailed ray tracing, Bayesian optimization employing Tree-structured Parzen Estimators (TPE)~\cite{} efficiently determines UAV placement. The optimization explicitly incorporates coherent communication metrics: channel capacity, SINR-based coverage, and fairness.

The instantaneous coherent channel capacity for UT $u$ at subcarrier $k$ under UAV configuration $\mathbf{X}$ is computed using Shannon's equation:
\begin{equation}
    C_{u,k}(\mathbf{X}) = B_{\text{sc}}\log_2\left(1 + \gamma_{u,k}(\mathbf{X})\right),
\end{equation}
where $B_{\text{sc}}$ is the subcarrier bandwidth. The total coherent achievable rate (sum capacity) across all covered UTs is given by:
\begin{equation}
    C_{\text{sum}}(\mathbf{X}) = \sum_{u\in\mathcal{U}_{\text{cov}}(\mathbf{X})}\sum_{k}C_{u,k}(\mathbf{X}).
\end{equation}

The optimization objective combines total coherent sum capacity, SINR-based coverage, and fairness, explicitly dependent on UAV configuration $\mathbf{X}$:
\begin{equation}
    \max_{\mathbf{X}}\; 
    \underbrace{C_{\text{sum}}(\mathbf{X})}_{\text{Sum Coherent Capacity}}\cdot
    \underbrace{\frac{|\mathcal{U}_{\text{cov}}(\mathbf{X})|}{|\mathcal{U}|}}_{\text{Coverage}}\cdot
    \underbrace{\frac{\left(\sum_b n_b(\mathbf{X})\right)^2}{N_b\sum_b n_b(\mathbf{X})^2}}_{\text{Fairness}},
\end{equation}
where $n_b(\mathbf{X})$ is the number of UTs served by UAV gNodeB $b$.

Additionally, UAV count optimization dynamically adapts based on Key Performance Indicators (KPIs). UAVs are iteratively added if SINR-based coverage or sum-capacity KPIs remain unmet:
\begin{equation}
    |\mathcal{B}| \leftarrow |\mathcal{B}| + 1,\quad \text{if}\quad \frac{|\mathcal{U}_{\text{cov}}(\mathbf{X})|}{|\mathcal{U}|} < \rho_{\text{target}},
\end{equation}
where $\rho_{\text{target}}$ denotes the targeted SINR-based coverage ratio. Conversely, redundant UAVs may be removed or repositioned if KPI thresholds are exceeded, ensuring optimized resource usage.

\subsection{Data Collection and Analysis Capabilities}
The DT framework provides comprehensive data, including coherent CIR samples, coherent MIMO IQ data, OFDMA scheduling logs, and Doppler spectrograms reflecting realistic mobility patterns.

These data enable robust analysis, performance assessment under mobility conditions, evaluation of advanced coherent communication algorithms, and support machine learning applications for proactive network management.

\subsection{Dataflow for Digital Twin based Disaster Relief}

The users continuously broadcast their locations and these are picked by LEO and UAV links. However they can calculate their locations with GPS, so it is not perfect locations. We assume they are in outdoors for the scope of this work. Data flow is given in figure \ref{fig:dt}

==> sections/unused/testbed_setup.tex <==
\section{Evaluation Methodology}
\label{sec:data_collection}

\subsection{Experiment Scenario}
Our experiments are conducted using a simulation environment based on the Sionna platform (v1.1), utilizing Python 3.12. We assume precise user equipment (UT) positions obtained through GPS, enabling accurate placement within the simulation scenario modeled on the San Francisco mesh (Figure~\ref{fig:sf_mesh}).  We also consider gNBs serving traditional cellular communication. The users are initially sampled from outdoor regions, verified via a bird's-eye view radio map, ensuring their positions remain valid and outdoors throughout subsequent perturbations. Once UAV are determined (as an example given in~\ref{fig:example_placement}), we simulate 100 slots of 5G downlink communication to evaluate performance under these spatial configurations. The primary simulation parameters utilized in our experiments are detailed in Table~\ref{tab:sim_parameters}. 

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.499\textwidth]{figures/sf_mesh.png}
    \caption{San Francisco simulation environment used for evaluating the TITAN framework. The mesh includes detailed building models and ground elevation variations to capture realistic urban topography. UTs are positioned 1.5 meters above the local ground surface to represent typical handheld device usage. {\color{red} Mention somewhere in the text and here that for this study we do not consider precise material properties -something like this.}}
    \label{fig:sf_mesh}
\end{figure}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.499\textwidth]{figures/example_placement.png}
    \caption{Example air-layer deployment in the TITAN framework. Small spheres represent UTs, while larger spheres indicate UAV positions. Each UT is color-coded according to its associated UAV; unassigned UTs are shown in gray. The ground plane displays the corresponding SINR-based coverage map. {\color{red} Should mark which ones are the UT/UAV etc... then merge with previous figure as two subfigures.}}
    \label{fig:example_placement}
\end{figure}

\begin{table}[ht]
\centering
\caption{Simulation Parameters}
\begin{tabular}{ll}
\hline
\textbf{Parameter} & \textbf{Value} \\
\hline
Carrier Frequency & 2 GHz \\
Subcarrier Spacing & 30 kHz \\
Number of Subcarriers & 660 (336 for D2C) \\
Number of OFDM Symbols & 12 \\
Transmit Power (BS, UAV) & 23 dBm \\
EIRP (D2C) & 85 dBm \\
BS Antenna Array & $4 \times 4$ Planar Array \\
UT Antenna Array & Single-element isotropic \\
Ray-Tracing Max Depth & 8 \\
Samples per TX & $10^8$ \\
Scheduler & Proportional Fair (PF) \\
Precoding & Regularized Zero-Forcing (RZF) \\
Post-Equalization & LMMSE \\
Noise Temperature & 290 K \\
Target TBLER & 10\% \\
\hline
\end{tabular}
\label{tab:sim_parameters}
\end{table}

\subsection{Disaster Scenarios}
To evaluate network resilience and recovery capabilities under disaster conditions, we simulate scenarios involving the progressive failure of infrastructure elements. Specifically, we consider three gNodeBs  and analyze how disabling each sequentially impacts the overall network performance. Additionally, we assess how effectively each competing method responds to such disruptions, examining network recovery dynamics and their ability to maintain service continuity amid partial infrastructure loss.

\subsection{Experiment Settings}
User terminals (UTs) are randomly selected exclusively from outdoor locations due to two primary reasons: (i) accurate modeling of indoor environments is not available in our simulation framework, and (ii) GPS signals typically exhibit unreliable behavior indoors. Once UT locations are set, we determine optimal UAV placements for the aerial communication layer. Subsequently, we perform detailed system-level simulations to evaluate downlink OFDMA performance comprehensively.

\noindent\textbf{System-Level Simulation and Protocol Stack:} Following UAV placements optimized by the DT (DT), we conduct system-level performance evaluations using \emph{Sionna SYS}. The simulation employs a protocol stack integrating proportional-fair (PF) scheduling, adaptive downlink power control, regularized zero-forcing (RZF) precoding, and linear minimum mean square error (LMMSE) equalization at the UT side.

Proportional-fair scheduling assigns coherent symbol streams dynamically, balancing instantaneous achievable data rates with historical throughput to maintain fairness across UTs. Downlink power control dynamically adjusts transmit power allocations according to instantaneous channel conditions and QoS demands, ensuring equitable resource distribution. Precoding for each subcarrier is performed using the RZF method, while UTs utilize coherent LMMSE equalization, optimizing symbol recovery by balancing noise suppression and interference mitigation.

The simulation runs over 100 OFDMA slots, iteratively performing these steps at each slot. Depending on hybrid automatic repeat request (HARQ) feedback, adaptive link adaptation is employed. Subsequently, key metrics, including the total number of transmitted bits, transport block error rate (TBLER), effective SINR values, and resource element (RE) assignments, are collected by the \name~framework.

\subsection{Competing Methods}
To rigorously evaluate the proposed TITAN method, we include comparisons against three other baseline approaches. The following benchmarks offer a comprehensive evaluation spectrum:

\noindent\textbf{Traditional D2C:}  
This baseline represents a direct-to-cell (D2C) scenario characterized by high elevation angles (30–45 degrees) and fewer subcarriers allocated to OFDMA, which boosts the link-level SNR. Due to limitations in ray-tracing distance and angular distribution from the low-earth-orbit (LEO) satellite, this method exclusively considers line-of-sight (LoS) links, representing the realistic constraints of traditional D2C deployments.

\noindent\textbf{Random UAV Placement:}  
This scenario serves as a performance lower-bound reference by deploying UAVs randomly within a 3D uniform spatial distribution throughout the target region.

\noindent\textbf{Bayesian Optimization (TR38.901):}  
To demonstrate TITAN's advantages comprehensively, this baseline leverages Bayesian optimization with the same objective function as TITAN but uses the stochastic 3GPP TR38.901 Urban Macrocell (UMa) model to estimate SINR values probabilistically, incorporating both LoS and non-line-of-sight (NLoS) probabilities.

\noindent\textbf{TITAN (Proposed Method):}  
Our proposed approach employs precise ray-tracing simulations for accurate and deterministic SINR estimation, enabling robust UAV placement optimization.

\subsection{Evaluation Metrics}
We evaluate performance differences among competing methods using two principal metrics: \textbf{sum-rate} and \textbf{coverage ratio}. Sum-rate quantifies the aggregate data throughput of all served users, directly reflecting overall network service quality. Coverage ratio measures the proportion of users successfully covered by the network, indicating the extent to which user demands are met under varying scenarios.

\subsection{O-RAN Testbed for Evaluation}
{\color{red} Noman}

Give the descriptions here.

% \section{Evaluation Methodology}
% \label{sec:data_collection}

% % \subsection{Real life?}
% % ADD DEPLOYMENT EXAMPLE and MESH

% \subsection{Experiment Scenario}
% Our experiments are conducted using Sionna-based simulations. We assume the user equipment (UT) coordinates are known via GPS, allowing precise placement within the simulation environment. The simulated scenario is based on the San Francisco mesh included in Sionna 1.1, running under Python 3.12 as given in figure \ref{fig:sf_mesh}. User locations are sampled from the outdoor regions of the radio map, which is generated using a bird's-eye view to ensure that users are positioned outdoors and not inside buildings. Perturbations to these initial locations are also constrained by this radio map, ensuring all users remain in valid positions throughout the simulation. Once user placements are finalized, we simulate the 5G downlink for 100 slots to evaluate the performance under these spatial configurations. The key simulation parameters are summarized in Table~\ref{tab:sim_parameters}.



% \begin{table}[ht]
% \centering
% \caption{Simulation Parameters}
% \begin{tabular}{ll}
% \hline
% \textbf{Parameter} & \textbf{Value} \\
% \hline
% Carrier Frequency & 2 GHz \\
% Subcarrier Spacing & 30 kHz \\
% Number of Subcarriers & 660 (336 for D2C) \\
% Number of OFDM Symbols & 12 \\
% Transmit Power (BS) & 23 dBm \\
% Transmit Power (UAV) & 23 dBm \\
% EIRP (D2C) & \textbf{85 dBm?} \\
% BS Antenna Array & $4 \times 4$ Planar Array \\
% UT Antenna Array & Single element, isotropic \\
% Ray-Tracing Max Depth & 8 \\
% Samples per TX & $10^8$ \\
% Scheduler & Proportional Fair (PF) \\
% Precoding & Regularized Zero-Forcing (RZF) \\
% Post-Equalization & LMMSE \\
% Noise Temperature & 290 K \\
% Target BLER & 10\% \\
% \hline
% \end{tabular}
% \label{tab:sim_parameters}
% \end{table}


% \subsection{Disaster Scenarios}

% In order to gauge the disaster damage to the infrastructure we also have 3 gNodeB in the simulations and going to measure how turning each of them will collapse the network slowly. Also we are going to see the disaster response with the competing methods + still active gNodeBs.


% \subsection{Experiment Settings}

% The UTs are randomly selected to be reachable outside locations, as we (i) do not have the the accurate interior building models, (ii) GPS does not work reliably. After this point UAV placement for Air layer is done. After that we do system level simulations to examine Downlink OFDMA performance. 

% \noindent{\bf System-Level Simulation and Protocol Stack: }
% Following the optimized UAV placement determined by the digital twin (DT), we evaluate system-level, coherent communication performance using \emph{Sionna SYS}. The implemented protocol stack includes essential functionalities such as proportional-fair (PF) scheduling, downlink power control, regularized zero-forcing (RZF) precoding, and coherent linear minimum mean square error (LMMSE) equalization at the UT receivers.

% PF scheduling dynamically assigns coherent symbol streams to resource elements (RE), maximizing the utility function defined as the instantaneous achievable coherent rate normalized by each user's historical throughput.

% Downlink power control is implemented to maintain fairness and meet minimum QoS requirements by allocating transmit power adaptively according to the channel conditions and user demands.

% The RZF precoding matrix at each subcarrier is used for precoding.

% At the UT receivers, coherent LMMSE equalization is employed to optimally recover the transmitted symbols, balancing interference suppression and noise mitigation.

% Using these methods we simulate 100 OFDMA slots. At each slot we do these stuff, then depending on the HARQ response we do link adaptation. \name then gathers number of bits sent, Ttransport block error rate (TBLER), effective SINR, OFDMA RE assignments for each slot.



% \subsection{Competing Methods}
% We compare 3 different methods, to fully evaluate TITAN's performance: 
% \begin{enumerate}
%     \item \textbf{Traditional D2C:} In order to illustrate how D2C falls short we use this method. This assumes 30-45 degree elevation angle with fewer number of subcarriers for OFDMA waveform to have more snr. We only consider LoS links for this method as SionnaRT only creates candidate rays uniformly and at 600km distance from the LEO satellite, only a handful of them reach the scene.
%     \item \textbf{Random:} In order to show performance lower bound we use random placement inside the area. The locations for UAVs are drawn from 3D uniform distribution.
%     \item \textbf{Bayesian (TR38.901):} In order to illustrate TITAN framework's gains meaningfully we also evaluate bayesian optimization which has the same optimization objective as TITAN, but it \textit{estimates} the SINR's through TR38.901 stochastic model UMA which considers LoS and NLoS probabilities.
%     \item \textbf{TITAN:} This is our proposed method that does raytracing based SINR calculation.
% \end{enumerate}

% \subsection{Evaluation Metrics}

% To grasp the differences we measure \textbf{Sumrate} and \textbf{coverage ratio} for each method. Sumrate is the summation of the data rate of all users and coverage ratio is coevered users. Sumrate allows us to gauge the quality of the service and covereage allows us to see how many users are satisfied.
